Robust Fair Clustering with Group Membership Uncertainty Sets

We study the canonical fair clustering problem where each cluster is constrained to have close to population-level representation of each group. Despite significant attention, the salient issue of having incomplete knowledge about the group membership of each point has been superficially addressed. In this paper, we consider a setting where the assigned group memberships are noisy. We introduce a simple noise model that requires a small number of parameters to be given by the decision maker. We then present an algorithm for fair clustering with provable \emph{robustness} guarantees. Our framework enables the decision maker to trade off between the robustness and the clustering quality. Unlike previous work, our algorithms are backed by worst-case theoretical guarantees. Finally, we empirically verify the performance of our algorithm on real world datasets and show its superior performance over existing baselines.

==> 04errormodels.tex <==
\section{Error Models and Problem Formulation}\label{sec:model_and_problem_statement}
\label{sec:error_models}
We introduce three families of error (noise) models and show that the first two models are special cases of the  generalized third model. For ease of representation we start with the simplest model, \emph{bounded aggregate error} (BAE), which only requires specifying a single noise parameter: the maximum number of points with incorrect memberships. While more elaborate models can potentially lead to solutions that exhibit lower degradation in the clustering cost, specifying only a single parameter eases the cognitive burden on a non-expert decision-maker. We then introduce the \emph{bounded pairwise error} (BPE) model which is more effective when the decision-maker has fine-grained information about the errors in the group memberships.  Specifically, there may be pairwise relationships known to a domain expert between groups $g, h \in \cH$, e.g., regarding the maximum number of points erroneously given membership $g$ when in fact they belong to $h$. We refer to this as \emph{error flow} from group $g$ to $h$.  Interestingly, we show that the BAE model is not actually a special case of the BPE model. Finally, we show that both models are special cases of the \emph{bounded aggregate and pairwise error} (BAPE) model, which combines parameters of both models: a bound on the total (aggregate) number of errors and the pairwise error between the groups. We formalize the relationships between these error models in \cref{obs:models}.

 % \SE{is flow the best word, should be consistent} \jpd{Removed it from the paragraph above; I don't think it's bad to use, though, gets the point across.}
 
Our models require the specification of a small number of parameters. In the case of the BAPE model which has the largest number of parameters, at most $1+ \ell (\ell-1)$ many parameters have to be specified where $\ell$ is the total number of groups.\footnote{Note that in many practical applications the number of groups can be very limited and in many well-motivated settings it can be as small as $2$ leading to at most $3$ parameters.} Further, the BAE model only requires specifying a single number. Moreover, the number of parameters that must be specified in all models does not grow as the size of the dataset (number of points) grows. This is a clear and significant advantage over the model of \citet{esmaeili2020probabilistic} which requires estimating the probabilistic membership information for each point which is a total of $\ell n$ many parameters. 
% \SE{below is my attempt to compare to Chabrax}
Furthermore, similar to \citet{Chhabra23:Robust} the BAE model imposes an upper bound on the number of points with incorrect group memberships. However, it has a clear advantage in that it does not need this set of points to be specified unlike \citet{Chhabra23:Robust}. Furthermore, the BPE and BAPE models give significant generalization and flexibility that is absent in \citet{Chhabra23:Robust}.  
% \SD{write a sentence about this parameter. How this parameter can be obtained etc. oth $m$ and $M$ can be learned. -- challenges in estimating these parameters?}

% \SE{this paragraph (Notation paragraph) does not flow well and I feel like it's just listing information}
\paragraph{Notation.} Prior to delving into the models, we introduce the parameters, and error quantities that are useful in describing our error models. 
All three error models are based on two error parameters namely, aggregate error $m$, and pairwise error $M$. Here $m$ denotes the maximum number of points with incorrect group memberships. 
The second parameter $M$ refers to an $\ell \times \ell$ pairwise error matrix which defines the error flow between any two groups $g,h \in [\ell]$. An entry $M_{g,h}$ in row $g$ and column $h$ refers to the maximum error that can flow from $g$ to $h$. Without loss of generality $M_{g,h}$ is at most $n_g$ where $n_g$ is the number points from group $g$ in the set $\cP$. Finally we make following assumptions on error models to avoid vacuous bounds: the error flowing out of group $g $ i.e., $\sum_{h}M_{g,h} < n_g$. 

Under a given model and a set of parameters, we define $\mgh$ as the maximum possible error flow from group $g$ to $h$ which is the maximum number of points from group $h$ that were falsely labeled as belonging to group $g$. Without loss of generality we can assume that $m_{h \rightarrow h}=0$ for any $h\in \cH$. We note that $\mgh$ can change based on the model but $M_{g,h}$ corresponds to the input parameter. 
The parameter $M$ imposes an upper bound restriction on the pairwise error flow from group $g$ to $h$. And in absence of such parameter, a natural restriction of $m$ is set by the \textit{aggregate error} parameter.  We fix the values of $\mgh$ for any pair of groups based on the error model and the parameters at hand. 


% \SE{send this to the beginning of the paragraph below}
% Both aggregate error $m$ and pairwise error matrix $M$ affect this error quantity $\mgh$. 
Similarly, we also define the maximum error \emph{inflow} and \emph{outflow} for any group. Let $\mhout$, and $\mhin$ represents \emph{positive error} and \emph{negative error} in any group.  Here the positive and negative error in a group $h$ corresponds to the maximum inflow error and maximum outflow error respectively. 
Moreover $\mhin$, and $\mhout$ cannot exceed $\sum_{g \neq h}n_g$ and $n_h$ respectively. The parameters $M$ and $m$ impose further restriction on the quantities $\mhin$, and $\mhout.$ These error quantities are crucial in determining the fairness violations for any group in a given clustering. 
% and \emph{negative error} or maximum error flow out of group $h$ respectively.
% mber of points falsely labeled as belonging to a group $g$ ($g \neq h$), but which actually belong to group $h$ 
 Finally, we let $\inm$ and $\outm$ denote the \emph{total positive error} ($\sum_{h}\mhout$) and \emph{total negative error} ($\sum_{h}\mhin$) across all the groups.
 The \emph{aggregate error}, denoted as $m^*$ is defined as the maximum possible error across all points, given by $m^*= \min\{\inm,n\}$.\footnote{This results from the straightforward observation that $\mhin$ equals $\mhout$.} We note that $m^*$ imposes an upper bound on the error quantities $\inm$, and $\outm$.

% \begin{fact}
%   Given a set of $n$ points with $\ell$ groups, we can say that  $\inm = \outm$ 
% \end{fact}
% Then, we can say that $\inm$ 
% Therefore, we can say that the \emph{negative} and \emph{positive} error for any group $h \in \cH$ is given by $\mhin $ 
% and $\mhout$ respectively. %= \sum_{g \in \mathcal{H}} m_{h \rightarrow g}$ 
% Let $\mh = \mhin + \mhout$ denote the \emph{total error} in group $h$ i.e., maximum number of points with false labels (inaccurate group memberships) related to group $h$. 
% \sd{edit this sentence again.}

% \emph{total positive error} (the sum of \emph{positive error} in any $h$ i.e., $\inm = \sum_{h}\mhin$) or the \emph{total negative error} (the sum of negative errors from each group $h \in [\ell]$ i.e., $\outm = \sum_{h}\mhout$ ).
% Therefore, we can say that 
% which is given by the total number of positive error.  
% Note that the aggregate error in BAE and BAPE models is specified as the model parameter. However, in the BPE model, the aggregate error can be defined as the minimum of \emph{total positive error\footnote{the sum of \emph{positive error} from each group $h \in [\ell]$ i.e., $\sum_{h \in \cH}\mhout$}} and \emph{total negative error\footnote{the sum of \emph{negative error} from each group $h \in [\ell]$ i.e., $\sum_{h \in \cH}\mhin$}}. This is because the aggregate error cannot exceed the overall \emph{false negatives} and \emph{false positives} in the membership assignments.

\paragraph{Bounded Aggregate Error model (BAE).} \label{sec:bae} In this model we are only given a single parameter, the \emph{aggregate error} $m$ which denotes the maximum permissible incorrect group memberships across all points. There is no information provided regarding the maximum error flow between any two groups. The main drawback in this model is that it allows the possibility of all $m$ inaccurate memberships occurring within a single group $h$, which may be too pessimistic, i.e., $\mgh := m$. In this model, there implicit restriction on the inflow and outflow errors $\mhin$, and $\mhout$ imposed by the aggregate error $m$ i.e., $\mhin:=m$ and $\mhout:=m$. Finally, the aggregate error is already given as an input parameter, i.e.,  $m^*:=m$. 

% Thus, we have $\mgh = \min\{m,n_g\}$ for all distinct $g,h \in \cH$ and $g \neq h$. 
% The second column of \cref{table:error_quantities} corresponds to relevant error quantities within the BAE model. 
% Since we know that $\mgh$ is the maximum error flow from groups $g$ to $h$, this quantity should be equal to $\mgh:=\min\{n_h,m\}$.
% where $n_h$ refers the total number of points in group $h$ . 
% Similarly, $\mhin$ is the maximum error flow into group $h$ which is equal to $\mhin:=\min\{ \sum_{g\neq h}n_g,m \}$ where $\sum_{g\neq h}n_g$ corresponds to the total number of points that do not belong to group $h$. 

%     \forall h, g \in \cH: \quad \mhg  &= \min\{n_h,m\} \label{eq:bae_start}\\
%   \forall h \in \cH, \quad  \mhout  &= \min\{n_h,m\} \\
%   \forall h \in \cH, \quad  \mhin &=  \min\{\sum_{g\neq h}n_g,m\} \\ 
%    m^*  &= m \label{eq:bae_end}
% \end{align}

\paragraph{Bounded Pairwise Error model (BPE).}  \label{sec:bpe}
% Given a $M (V,E,\{\mgh\}_{(g,h)\in E})$ representing bounded pairwise error misidentifications between groups, where the vertices $V$ correspond to groups. Each directed edge $(g,h)$ is associated with an integer $\mgh$ signifying the maximum number of points from group $g$ who were erroneously identified as belonging to group $h$. 
% In this model we assume that we are given a $\ell \times \ell$ matrix $M$ where $\mgh$ is the entry in row $g$ and column $h$, which is the maximum number of points from group $g$ who were erroneously identified as belonging to group $h$. A main distinction from the \textit{aggregate} model is that we can model additional nuances within groups and need not assume arbitrary noisy within groups.  
In this model, we are given the \textit{pairwise error matrix} $M$ defined as above, therefore, we have $\mgh:= M_{g,h}$. Since there is no explicit restriction on inflow and outflow of any group $h$, we have $\mhin := \sum_{g}\mgh  $ and $\mhout:= \sum_{g}\mhg$.  
A key difference from the \emph{bounded aggregate error} model is that we can capture more intricate details within groups, eliminating the need to assume an overly pessimistic pairwise error flow for any pair of groups. However, it is important to highlight that this model places no restriction on the \emph{aggregate error} $m^*$---the total number of noisy labels across all the points i.e., $m^*:=\inm=\sum_{h}\mhin.$ 
% Precisely, this quantity can be as large  represents the \emph{total positive error} or the \emph{total negative error}. 
% This is because the aggregate error cannot exceed the total number of \emph{false negatives} or \emph{false positives} across all the points.  
% \begin{align}
%     \forall h,g \in \cH ,\quad \mhg &= \min\{M_{g,h},n_h\}   \label{eq:bpe_start} \\ %%\text{\sd{Is this constraint necessary?}}
%      \forall h \in \cH ,\quad \mhout &= \min\{\sum_{g\neq h}\mhg,n_h\} \\
%       \forall h \in \cH ,\quad \mhin &= \min\{\sum_{g\neq h}\mgh,\sum_{g\neq h}n_g\} \\ \label{eq:bpe_end}
%         m^* &= \min\{ \inm,n \}
% \end{align}

 This model can be further generalized by introducing an additional parameter $m$, representing  the \emph{aggregate error} allowed. This extension leads to a more general model called \emph{Bounded Aggregate and Pairwise Error Model} (BAPE) defined as follows.


% \begin{table}[h!]
% \centering
% \scalebox{0.86}[0.86]{
% \ra{1.3}
% \begin{tabular}{l|lll}
%  \hline  
% \begin{tabular}{@{}lll@{}} {Error Quantity}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAE}  \end{tabular} & \begin{tabular}{@{}c@{}}{BPE}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAPE}  \end{tabular} \\
%  \hline
%   $\mhg$ & $\min\{n_h,m\}$ & $\min\{n_h,M_{g,h},\}$ & $\min\{n_h,M_{h,g},m\}$ \\ 
%  $\mhout$ & $\min\{n_h,m\}$ & $\min\{\sum_{g\neq h}\mhg,n_h\}$ & $\min\{\sum_{g\neq h}\mhg,n_h,m\}$ \\ 
%  $\mhin$ & $ \min\{\sum_{g\neq h}n_g,m\}$ & $\min\{\sum_{g\neq h}\mgh,\sum_{g\neq h}n_g\} $ & $\min\{\sum_{g\neq h}\mgh,\sum_{g\neq h}n_g,m\} $ \\ 
%  $m^*$ & $\min\{m,n\}$ & $\min\{\inm,n\}$ & $\min\{m,n\}$ \\ \hline
% \end{tabular}}
% \vspace{0.3cm}
% \caption{ For parameters $m$ and $M$ given, we define $\mgh$ as the maximum error flow from group $g$ to $h$. The quantities $\mhin$ and $\mhout$ represent the maximum error flow into and out of each group $h$ respectively. Additionally, $m^*$ corresponds to the total number of errors across all points. \SE{I think the writing should be clear so that the table is not needed.}}
% \label{table:error_quantities}
% \end{table}


\paragraph{Bounded Aggregate and Pairwise Error model (BAPE).\label{sec:bape_model}} 
The general model is characterized by both {aggregate error} $m$ and pairwise error matrix $M$. This model more accurately depicts the error quantities using information from both the parameters. The error flow from group $g$ to $h$ is $\mgh:= \min\{M_{g,h}, m\}$. The error inflow and outflow  for any group $h\in [\ell]$ has an implicit restriction similar to the aggregate error i.e., $\mhin:=\min\{\sum_{g}\mgh,m\}$ and $\mhout:=\min\{\sum_{h}\mhg,m\}$. Finally, we have $m^*= m$.  
% \SE{I think there is a minimum missing in the last two assigments} 

We make two simple observations :  (1) BAE model with only an aggregate error $m$ is a special case of BAPE model where the pairwise matrix $M$ can be defined as follows: $M_{g,h}:= m$ for any $g,h \in \cH$ and $g \neq h$. (2) BPE model with a single error parameter $M$ is also a special case of BAPE model with the error parameters $m^* = \sum_{h \in [\ell]} \sum_{g\in [\ell]} \min\{M_{g,h}, n_g\} $ and $M$. However, BAE cannot be directly modeled as BPE, and vice versa. We formalize this as follows.
% Notice that both error models BAE and BPE can be formulated to special cases of the BAPE model. 
\begin{lemma} \label{obs:models}
Both the error models \emph{BAE} and \emph{BPE} are special cases of \emph{BAPE} while neither is a special case of the other. \end{lemma}

% Any given parameters $(m,M)$, the \emph{total error\footnote{the sum of poisitive and negative error i.e., $m_h = \mhout + \mhin$}} associated with any group is at most $m$ i.e., $\mh \leq m.$

% must satisfy the following constraints (i) the positive error, and negative error associated with any group $h$ is at most $m$, and (ii) the total error 
% ($g \neq h$) is at most $m$, (ii) the total number of points that flow out of $h$ from any group $g$ ($g \neq h$) is at most $m$, 
% formulated below.
% \begin{equation*} 
%     \mhin = \sum_{g \neq h}\mgh \leq  m, \mhout = \sum_{g \neq h}\mhg \leq m, \mh  = \max \big\{\mhin + \mhout,m\big\}  
% \end{equation*}
% \SE{The upper definition is circular!!! Can't you just say $\mhin, mhout \leq m$???}
% These inequalities guarantee that the maximum number of \emph{false negatives} and \emph{false positives} i.e., total error in any group $h\in\cH$ does not exceed the aggregate error $m$.   
\begin{example} \label{ex:toy_ex}
    Consider a toy example containing two red and two blue points. Following figure shows all possible memberships, under BAE, BPE, and BAPE models with aggregate error $m=2$ and pairwise error matrix $M$ with $M_{r,b} = 1$, and $M_{b,r}=2$.
\end{example}
% \begin{table}[h!]
% \centering
% \scalebox{0.95}[0.95]{
% \ra{1.3}
% \begin{tabular}{l|lll}
%  \hline  
%  \begin{tabular}{@{}lll@{}} {Error Quantity}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAE}  \end{tabular} & \begin{tabular}{@{}c@{}}{BPE}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAPE}  \end{tabular} \\
%  \hline
%   $m_{r\rightarrow b}, m_{b \rightarrow r} $ & $2,2$ & $1,2$ & $1,2$ \\ 
%  $m_{r \rightarrow}, m_{b \rightarrow}$ & $2,2$ & $1,2$ & $1,2$ \\ 
%  $m_{ \rightarrow r}, m_{\rightarrow b}$ & $2,2$ & $2,1 $ & $2,1$ \\ 
%  $m^*$ & $2$ & $3$ & $2$ \\ \hline
% \end{tabular}}
% \vspace{0.3cm}
% \caption{ For parameters $m$ and $M$ given, we define $\mgh$ as the maximum error flow from group $g$ to $h$. The quantities $\mhin$ and $\mhout$ represent the maximum error flow into and out of each group $h$ respectively. Additionally, $m^*$ corresponds to the total number of errors across all points. }
% \label{table:error_quantities}
% \end{table}

% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.45]{Figures/final_models.png}
%     \caption{The figure depicts all feasible memberships for the toy instance on the left, consisting of $2$ red and $2$ blue points, under BAE, BPE, and BAPE models with $m=2$ and $M=\begin{bmatrix}
% 0 & 1 \\
% 2 & 0 \end{bmatrix}.$ Feasible sets for BAE, BPE, and BAPE are highlighted in red, purple, and green respectively.}
%     \label{fig:final_model}
% \end{figure}


%  \begin{figure}[!ht]
%     \centering
%    \includegraphics[scale=0.3]{Figures/final_models.png}
%     \quad
% \scalebox{0.7}[0.7]{
% \ra{1.3}
% \begin{tabular}{l|lll}
%  \hline  
%  \begin{tabular}{@{}lll@{}} {Error Quantity}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAE}  \end{tabular} & \begin{tabular}{@{}c@{}}{BPE}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAPE}  \end{tabular} \\
%  \hline
%   $m_{r\rightarrow b}, m_{b \rightarrow r} $ & $2,2$ & $1,2$ & $1,2$ \\ 
%  $m_{r \rightarrow}, m_{b \rightarrow}$ & $2,2$ & $1,2$ & $1,2$ \\ 
%  $m_{ \rightarrow r}, m_{\rightarrow b}$ & $2,2$ & $2,1 $ & $2,1$ \\ 
%  $m^*$ & $2$ & $3$ & $2$ \\ \hline
% \end{tabular}}
%     \captionlistentry[table]{A table beside a figure}
%     \captionsetup{labelformat=andtable}
%     \caption{For parameters $m$ and $M$ given, we define $\mgh$ as the maximum error flow from group $g$ to $h$. The quantities $\mhin$ and $\mhout$ represent the maximum error flow into and out of each group $h$ respectively. Additionally, $m^*$ corresponds to the total number of errors across all points.}
%   \end{figure}

% The figure depicts all feasible memberships for the toy instance on the left, consisting of $2$ red and $2$ blue points, under BAE, BPE, and BAPE models.
  \begin{minipage}{\textwidth}
  \begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[scale=0.35]{Figures/Final_Ex.png} 
    \captionof{figure}{Feasible sets for BAE, BPE, and BAPE are highlighted in red, purple, and green respectively for \cref{ex:toy_ex}. \label{fig:final_model}}
  \end{minipage}
  \end{minipage}

 \begin{minipage}[b]{0.44\textwidth}
    \centering
    \ra{1.3}
{
\scalebox{0.8}{%
\begin{tabular}{l|lll} 
 \hline  
\begin{tabular}{@{}lll@{}} {Error Quantity}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAE}  \end{tabular} & \begin{tabular}{@{}c@{}}{BPE}  \end{tabular}& \begin{tabular}{@{}lll@{}}{BAPE}  \end{tabular} \\
 \hline
 $\mrb,  \ \mbr  $ & $2,2$ & $1,2$ & $1,2$ \\ 
 $\mrto, \ \mbto $ & $2,2$ & $1,2$ & $1,2$ \\ 
 $\mtor, \ \mtob $ & $2,2$ & $2,1 $ & $2,1$ \\ 
 $m^*$ & $2$ & $3$ & $2$ \\ \hline
\end{tabular}%
}%end of scalebox
\vspace{0.52cm}
      \captionof{table}{The error quantities related to the maximum error flow between any two groups, as well as the inflow and outflow for each group.}}
    \end{minipage}
  \end{minipage}
% We refer the reader to a clean proof in Appendix~\ref{sec:ommitted_proofs}. \SE{remove this, instead somewhere early say that all proofs are delayed to the appendix}.

% The objective is to identify a clustering of points that remains \textit{robust} in the presence of these $m$ noisy memberships. We formalize the definition of robustness in section~\ref{subsec:problem_formulation}.

% indicating the group memberships of points and a directed graph $G$ that contains the bounded bounded pairwise error error noisy memberships. 

% Our rationale for this choice is as follows, (i) Any two groups $g,h \in \cH$ can either be confused with but some groups are uncorrelated hence the chance of such noisy memberships is very low, (ii)




% A model that unifies both \textit{bounded aggregate error} and \textit{bounded pairwise error noisy memberships} has an budget $m$ which is the maximum number of points with noisy labels while still allowing for the bounded pairwise error correlated noise information via the matrix $M$. Additionally for each group $h \in \cH$ we modify $\mhin(\mhout)$ as $\mhin = \min\{\mhin,m\}(\mhout = \min\{\mhout,m\})$ since the maximum number of misidentifications of any group cannot exceed the budget $m$.
% we let $\mhin$ and $\mhout$ denote the quantities $\sum_{g}\mgh$, and $\sum_{g}\mhg$ respectively. $(f_s,\{c_e\}_{e\in E_G})$

% \paragraph{Flow network to represent our models.} Here we give a flow network (see Figure~\ref{fig:flownetwork}) representation of our noisy membership models described above. Let $\cG = ( I \cup J \cup \{s,s',t,t'\} ,m,M)$ where $m$ is the flow out of the source $s$, set of vertices $I$($J$) corresponds to each group $h \in \cH$ i.e., $I= \{ i_h\}_{h\in \cH}(J= \{ j_h\}_{h\in \cH})$, and $M$ is the capacities on the edges between $I$ and $J$ i.e., $c(i_g,j_h) = \mgh $ for each $g ,h \in \cH$. The flow in each edge $f_{e}$ for each edges $\{ e =  (s',i_g)\}_{g\in \cH}$$\Big(\{ e =  (j_g,t')\}_{g\in \cH}\Big)$ represents the number of false positives (true negatives) in group $g$. Additionally, through each edge $e = (i_g,j_h)$ represents number of points that are misclassified as $g$ but originally belong to group $h$. 


% . {Aggregate:} $(m,\{c_{g,h}:m\})$, Pairwise:~$(m^*,\{c_{g,h}:\mgh\}),${Unified model} : $(m,\{c_{g,h}: \min\{m_{g,h},m\})$.}

==> conclusion.tex <==
\section{Conclusion}
\SE{maybe remove if there is not enough space}
